Road Friction Estimation for Connected Vehicles using Supervised Machine Learning

In this paper, the problem of road friction prediction from a fleet of connected vehicles is investigated. A framework is proposed to predict the road friction level using both historical friction data from the connected cars and data from weather stations, and comparative results from different methods are presented. The problem is formulated as a classification task where the available data is used to train three machine learning models including logistic regression, support vector machine, and neural networks to predict the friction class (slippery or non-slippery) in the future for specific road segments. In addition to the friction values, which are measured by moving vehicles, additional parameters such as humidity, temperature, and rainfall are used to obtain a set of descriptive feature vectors as input to the classification methods. The proposed prediction models are evaluated for different prediction horizons (0 to 120 minutes in the future) where the evaluation shows that the neural networks method leads to more stable results in different conditions.

==> include/Proposed.tex <==



\subsection{Evaluate the datasets}
To evaluate whether some proposed feature set seems promising we'll use two exploratory data analysis tools, PCA and t-SNE. These dimension reducing algorithms are good at revealing any possible internal structure of the data. These will give us an indication of the amount of important information there is in the dataset. \\
But first, we'll draw a correlation matrix of the different features we are evaluating. As seen in the graph there are some correlated features.
\begin{figure}[H]
\centering
\includegraphics[width=13cm]{figure/corr_matrix.png}
\caption{A correlation matrix with the available the features.}
\end{figure}
It seems that we have a solid correlation between the friction value and the air humidity, the amount of rain and the previously measured friction values.

To visualize the dataset we run the PCA algorithm on the dataset to reduce the original number of features down to two. This is done to visualize the whole dataset in one graph.
\begin{figure}[H]
\centering
\includegraphics[width=12cm]{figure/PCA.png}
\caption{PCA dimensionality reduction over original features.}
\end{figure}
This technique is used to find any abnormal datapoints which we need to exclude before doing any further analysis.

In addition to PCA we'll another dimensionality reduction method called  
t-Distributed Stochastic Neighbor Embedding (t-SNE). Here, t-SNE will be used for visualization of high-dimensional data which is its primarily use case. It has a useful property not found in PCA; t-SNE is nonlinear and acts on the probability of two points being selected as neighbours. This is described in detail in the chapter three.
\begin{figure}[H]
\centering
\includegraphics[width=12cm]{figure/t-SNE.png}
\caption{t-SNE embedding over the features.}
\end{figure}
In this graph we can observe local clusters of data points. This gives us a good a indication that the dataset has some inner structure. We'll do this analysis with different datasets from all the road segments to try identifying the most important features. It is worth to notice that since t-SNE is stochastic, multiple runs will produce different embeddings.


\section{Preprocessing}
Before we train the models the dataset will be normalized so that  it has zero mean and unit variance. By adjusting values measured on different scales to a notionally common scale each feature will be of same importance.


\section{Dimensionality Reduction}
The goal of reducing the dimensionality of a dataset is to reduce the dimension while still minimizing the loss of important information. In this project we'll apply PCA as a tool for dimensionality reduction. PCA does not infer any prior knowledge of what information is important. It is just based upon the variation of the data itself. It finds orthogonal basis of the data with basis vectors which are sorted by the amount of variance in their direction. With this technique we can extract the subspaces that accounts for a known amount of variance. We can set a threshold for the amount of variance we want to extract or just set a maximum number of dimensions. PCA extracts a linear subspace which we then use as as the feature set.
Our assumption is that subspaces with lower variances will represent the information which are not changing as much as the other subspaces and might therefore be less important. Finding a good threshold between useful data and noise varies from case to case. In this analysis we'll use a combination of looking at the results and using t-SNE to find a suitable maximum number of dimensions or a threshold for the variance.
In this project we'll apply the PCA algorithm before we train the Logistic Regression and the SVM models. In principal, the linear transformation performed by PCA can be performed just as well by by the input layer weights of the neural network, so it isn't strictly speaking necessary to use PCA for the neural network. However, as the number of weights in the network increases, the amount of data needed to be able to reliably determine the weights of the network also increases and overfitting becomes more of an issue.\\
The benefit of dimensionality reduction is that it reduces the size of the network, and hence the amount of data needed to train it. The disadvantage of using PCA is that the discriminative information that distinguishes one class from another might be in the low variance components, so using PCA can make performance worse when traning the neural network.


\section{Classification}
After having reduced the feature set we're at the stage where we want to train our models with supervised learning. For each of the three road segments we're train and evaluate each of the classifiers.

\subsection{Logistic Regression}
In this project we'll use a binary logistic regression classifier. The binary logistic model is used to estimate the probability of a binary response based on a predictor. In this case will we try to predict if the road is slippery or not. The predicted values are probabilities and are therefore restricted from zero to one through the logistic distribution function because logistic regression predicts the probability of particular outcomes.

\subsection{Support Vector Machine}
As mentioned in chapter three, a Support Vector Machine (SVM) is a discriminative classifier formally defined by a separating hyperplane. From labeled training data, the algorithm outputs an optimal hyperplane which categorizes new examples. Here, soft-margin is used to improve the results. When training the models the non-linear kernel called Radial basis function were utilized.




\subsection{Artificial Neural Network}
As mentioned in the theory chapter, an neural network can be varied in many ways. For this project we decided to use one hidden layers. The hidden layer contains the same number of nodes as inputs in the input layer. Since we have a smaller training set more layers and nodes would cause overfitting problems. In the next chapter we did an evaluation of how more hidden layers effected the results.\\
Before each training session all weights were set to a random number between -0.1 and 0.1. We found that relu activateion function worked best with our datasets. This activation functions were chosen due to the nature of min-max normalization and due to results from Glorot et al. \cite{relu}. Even though the rectifier activation function isn't continious below zero, blocking the gradient back-propagation is part of rectifier advantage.\\
To avoid training models that were overfitted, the networks with the lowest evaluation error was stored. At the output layer we applied a linear activation function. Since this results in values from everything in between 0 and 1 we applied a threshold filter to get the prediction.


\section{Cross Validation}
All models have been assessed through k-fold cross validation and due to stochastic elements in the evaluation process different runs of the algorithm might yield different results. Therefore we run the tests, with the same hyperparameters, several times and take the average. Since we need to run the evaluation code several times this is a very computationally demanding task for the neural network. So instead of evaluating all combinations of features and hyperparameters, we'll do an estimation of which features and  hyperparameters works best. We perform a small variation for key hyperparameters or feature sets to get an insight into which setup works best. 

%\section{Post processing}


==> include/Theory.tex <==
% CREATED BY Erik Ek, 2016
\chapter{Theory}

The chapter will give an general insight into the general methods and concepts of the techniques used in this project. The actual implementation of these methods will be discussed in chapter four.


\section{Classification}
In statistics and machine learning, classification is the problem of predicting to which of a set of categories a new observation belongs, on the basis of a training set of data containing observations whose category membership is known. Classification can imply two separate methods – binary classification and multiclass classification. In binary classification, which we'll apply, only two outcomes are involved. Whereas multiclass classification involves assigning an object to one of several classes. Classifiers performance depends greatly on the characteristics of the data to be classified, we are therefore trying three different classifiers in this project.\\
In this report error rate, sensitivity and selectivity will be used as metrics to evaluate the quality of these three classification medthods.

\section{Logistic Regression}
Logistic regression is a technique in statistics to build a model that is aimed at finding the best fitting and most accurate and sensible model to assess the relationship between a set of responsive variables and at least one explanatory variable. It differs from the linear regression in that it can be applied when the dependent variable is categorical and doesn't require rigorous assumptions to be met.

\subsection{Binary Logistic Regression}
Binary logistic regression is a prognostic model that is fitted where there is a binary dependent variable like in this instance where we are interested in whether a road surface is slippery or not. The categories are usually coded as 0 and 1 as it results is a straightforward interpretation.

\subsection{Logistic Regression Model}
We have some independent observations $y_1,\dots,y_m$. These can be treated as realizations of a random variable with the binomial distribution with probability $\pi_i$ for every observation $i$. We suppose that the logit of the underlying probability $\pi_i$ is a linear function of the predictors $\text{logit}(\pi_i)=x_i'\beta$ where $x_i$ is a vector of covariates and $\beta$ a vector of regression of coefficients. This defines a generalized linear model with link logit and binomial response.\\
The logistic regression model is given by
\[
\pi(x_i)=P(y_i=1;x_i)=(1+e^{-X^T\beta})^{-1}
\]
where $y_i$ is 1 if the friction is high and 0 if the friction is low for all $i$. $\pi(x_i)$ is the probability of an event that depends on p-independent variables. We can rewrite this as
\[
1-\pi(x_i)=1-\frac{1}{1+e^{-X^T\beta}}=\frac{(1+e^{-X^T\beta})-1}{1+e^{-X^T\beta}}=\frac{e^{-X^T\beta}}{1+e^{-X^T\beta}}
\]
which gives us that
\[
\frac{\pi(x_i)}{1-\pi(x_i)}=\frac{1}{e^{-X^T\beta}}
\]
Thus
\[
\text{ln}\left(\frac{\pi(x_i)}{1-\pi(x_i)}\right)=\text{logit}(\pi(x_i))=X^T\beta
\]
This classifier quantifies the relationship between the dichotomous dependent variable and the predictors using odds ratios. Odds ratio is the probability that an event will occur divided by the probability that the event will not happen. 
Odds are calculated using the formula
\[
\frac{\pi(x)}{1-\pi(x)}
\]
where $\pi(x)$ is the probability of success and $(1-\pi(x))$ is the probability of failure. 

\section{Support Vector Machine Classification}
In this case we'll train support vector machines (SVM) with only two classes. We consider a data set $\omega = {(x_1,y_1),(x_2,y_2),\dots,(x_n,y_n)}$ where $x_i\in \mathbb{R}^d$. $x_i$ is the feature set of the i:th input pattern. When using the SVM we can create a nonlinear decision boundary by transforming the data by a non-linear function to a higher dimensional space. The data points are then moved from the original space $I$ onto a feature space we call $F$. \\
The goal of the algorithm is to find a hyperplane which is represented with the equation $w^Tx+b=0$ where $w\in \mathbb{R}$. The hyperplane determines the margin between the classes. Ideally we are looking for a hyperplane that can separate the two classes of data by maximizing the distance from the closest support vectors from each class of the hyperplane is equal; thus the constructed hyperplane searches for the maximal margin. One trick consist of using a soft margin to prevent overfitting noisy data. It's a regularization technique that controls the trade-off between maximizing the margin and minimizing the training error.\\
We introduce a slack variable $\xi_i$ that allows some data points to lie within the margin, and a constant $C>0$ which determines the trade-off between maximizing the margin and the number of support vectors within that margin.
\begin{figure}[H]
\centering
\includegraphics[width=9cm]{figure/SVM_2.png}
\caption{An example of an support vector machine classifier with soft margin. The hyperplane ($w^Tx+b=0$) is separating the two data classes in these two dimensions with some margin of error.}
\end{figure}
When training a SVM classifier we use the following loss function
\[
\text{min}\frac{||w||^2}{2}+C\sum^n_{i=1}\xi_i
\]
which are subject to: $y_i(w^T\phi(x_i)+b)\geq1-\xi_i$ $\forall i=1,\dots,n$ and $\xi_i\geq0$ $\forall i=1,\dots,n$.
The minimization problem is solved using Lagrange multipliers and we get
\[
f(x)=\text{sgn}\left(\sum_{i=1}^n \alpha_i y_i K(x,x_i)+b\right)
\]
where $\alpha_i$ are the Lagrange multipliers. Every $\alpha_i$ is weighted in the decision function and thus supports the so called machine. SVM is spares and therefore there will be few Lagrange multipliers with a non-zero value.

\subsection{Kernel function}
We introduce the kernel function $K(x,x_i)=\phi(x)^T\phi(x_i)$ which only relies on the dot product of the vectors in feature space $F$. When using a kernel it's not necessary to perform an explicit projection to that space as long as the function $K$ has the same results. It can be used instead. This is called the kernel trick. The feature space $F$ can have unlimited dimensions and the hyperplane separating the data can be very complex. This is what gives the SVM its ability to separate non-linear separable data points. One of the popular kernels is the Gaussian Radial Basis function defined as
\[
K(x,x')=\text{exp}\left(-\frac{||x-x'||^2}{2\sigma^2}\right)
\]
$||x-x'||$ is the dissimilarity measure and the $\sigma$ is a kernel parameter. One of the greatest advantages of this method lies in its applicability in almost any dimension because of its versatility. There are generally little restrictions on the way the data are prescribed.



\section{Artificial Neural Networks}
In this section, the theory behind multilayered perceptron neural networks will be explained. Since we have a supervised classification problem; we are given a set of training pairs $(x,y),x\in X,y\in Y$ and we try to find a function such that $f:X\to Y$. We wish to infer the mapping implied by the data. Artificial neural networks consist of neurons which are the building blocks of the network. Here is a example of a neuron connected with inputs and a bias.

\begin{figure}[H]
\centering
\includegraphics[width=9cm]{figure/neuron.png}
\caption{We have a set of connecting inputs ($x_1,x_2,\dots,x_j$), each connected to there own weight ($w_{k1},w_{k2},\dots,w_{kj}$). The input is multiplied by the synaptic weight and added together with the bias term ($b_k$). This operation is a linear combiner. After the sum is calculated we apply an activation function ($\varphi$) on the signal and get an output $y_k$ where the amplitude is limited.}
\end{figure}

The bias input is increasing or decreasing the net input of the activation function depending on whether its positive or negative.
\\
This output can be expressed with the following equation
\begin{equation}
y_k= \varphi\left(\sum^m_{j=1}w_{kj}x_j+b_k\right)
\label{fig:first_lion}
\end{equation}

The activation function, $\varphi$, defines the shape of the output of a neuron. We can add the bias term and the equation could be written as
\begin{equation}
y_k= \varphi\left(\sum^m_{j=0}w_{kj}x_j\right)
\label{fig:lion}
\end{equation}

where a new so called synapse have been added. In neural networks, a synapse could be described as a connection between two neurons. Corresponding in biology to the amount of influence the firing of one neuron has on another. In \ref{fig:lion} above we set $x_0=1$ and then let the weight term $w_{k0}=b_k$. We now account for the bias term and can reformulate the model with $x_0$ as an regular input.

\subsection{Activation functions}
There are many different activation functions which have thier own use cases. The simplest one is the threshold function which is defined as
\[
\varphi(p) =
\begin{cases}
0 & \text{if } p<0,
\\
1 & \text{if } p\geq 0,
\end{cases}
\]

One other popular activation function is the sigmoid function which is mathematically defined as
\[
\varphi(p) = \frac{1}{1+e^{-cp}}
\]
where c is the slope parameter. The sigmoid function is differentiable which makes it useful when we are training the network. More on that later. The sigmoid function is also a bounded differentiable real function that has a positive derivative at each point. The threshold function and sigmoid function limit the output within zero and one.
In our implementation we'll use the widely used rectifier activation function which is defined as $\varphi(p)=\text{max}(0,p)$. This function could be approximated as the smooth analytic function $\varphi(p)=\text{ln}(1+e^p)$.
\begin{figure}[H]
\centering
\includegraphics[width=12cm]{figure/activation_funcs.png}
\caption{Here are plots of some of the activation functions that we are utilizing in this project.}
\end{figure}
However, it is sometimes suitable to have a activation function that can limit the output within $[-1,1]$. For this the signum function or hyperbolic tangent can be useful. The signum function is just like the threshold function but goes from -1 to 1 like a step function.


\subsection{Network Architecture}
The structure we'll use is a multi layered feedforward network. This network is characterized by one or more hidden layers. The layers consist of neurons which we call nodes. The input layer forwards the input to the nodes and passes the outputs to the hidden layer. The hidden layer then forwards the input from the input layer to the output layer. By applying a technique called backpropagation we change the weights in these neurons to minimize the output from a cost function. Each nodes will try to find structures of the data fed to them. There is no limits on the number of neurons or hidden layers one can use. Each input node represents a feature in the input set.
\begin{figure}[H]
\centering
\includegraphics[width=8cm]{figure/Network.png}
\caption{The nodes (circles) represents the neurons. Each node is connected to the other nodes in the next layer. Each node will also have a bias input connected to it which is not shown in this graph.}
\end{figure}
In this project we will utilize a multi layered feedforward network with at least one hidden layer. The alternative is to use a single layered feedforward network where the input layer projects its output directly onto an output layer without any hidden layers. A common problem that can occur if we train a network with too many layers or nodes is overfitting. Therefore we'll try to find the right amount of complexity for the network.

\subsection{The Backpropagation Algorithm}
To train the network we use a technique called backpropagation. This is the most common algorithm for training a multilayer perceptron neural network. The algorithm updates the weights between the nodes of the network by applying an optimization algorithm. A popular such optimizer is the gradient descent which is commonly used. However, there are other such algorithms that could, in some cases, be used for better results. One popular such algorithm is the Stochastic Gradient Descent (SDG). We'll try a variant of SDG called Adam optimizer, which is widely used to minimize the error rates in neural networks successfully.

\subsection{The Cost Function}
To improve our model we try to minimize a the output from a cost function which is related to the mismatch between our mapping and the data and it implicitly contains prior knowledge about the problem domain. We assume a smooth cost function $E(\bar{w})$ where $\bar{w}$ is a weight vector. Then the cost function is a indication of how to change the weight values in the network so we will find an optimal solution. 
In this project we used softmax cross entropy with logits as the cost function. The cross entroy is frequently used in optimization estimation. The cross entroy cost function is defined as
\[
H(X,Y) =  y^{(i)}\text{ln}(a(x^{(i)})+\left(1-y^{(i)}\right)\text{ln}\left(1-a(x^{(i)})\right)
\]
where $X=\{x^{(1)},\dots,x^{(n)}\}$ is the set of input values and $Y=\{y^{(1)},\dots,y^{(n)}\}$ is the corresponding set of labels for those input examples. $a(x)$ represents the output of the neural network given input $x$. Each of $y$ is either 0 or 1, and the output function $a$ is restricted by the interval 0 to 1 as well. The crucial thing to note is that softmax cross entropy with logits performs an internal softmax on each row of logits so that they are interpretable as probabilities before they are fed to the cross entropy equation. %Then, let $x_{\text{logits}} = \text{logits}$ and the softmax cross entropy with logits cost is defined as
%\[
%H'(X,Y) = y^{(i)}\text{ln}\left(\text{sigmoid}(x^{(i)}_{\text{logits}})) + (1 - y^{(i)}\right) -\text{ln}\left(1 - \text{sigmoid}(x_{\text{logits}}^{(i)})\right)
%\]
%= z * -log(1 / (1 + exp(-x))) + (1 - z) * -log(exp(-x) / (1 + exp(-x)))
%= z * log(1 + exp(-x)) + (1 - z) * (-log(exp(-x)) + log(1 + exp(-x)))
%= z * log(1 + exp(-x)) + (1 - z) * (x + log(1 + exp(-x))
%= (1 - z) * x + log(1 + exp(-x))
%= x - x * z + log(1 + exp(-x))

\subsection{Gradient Descent}
For every iteration we want to find a solution $\bar{w}^*$ such that $E(\bar{w}^*)\leq E(\bar{w})$. The gradient descent algorithm updates the weight vector $\bar{w}$ is the opposite direction of the gradient vector $\nabla E(\bar{w})$. We introduce a learning rate $\eta$ and define the algorithm as
\[
\bar{w}(n+1)=\bar{w}(n)-\eta\nabla E(\bar{w})
\]
and if we are going from $n$ to $n+1$ this can be defined as
\[
\Delta \bar{w}(n)=\bar{w}(n+1)-w(n)=-\eta \nabla E(\bar{w})
\]
We have a multilayer perceptron neural network with one or more hidden layers, and an output layer. The error signal produced at the output of neuron $i$ is given by $e_j(n)=d_j(n)-y_j(n)$. Which gives us the error between the network output $y_j(n)$ and the desired response $d_j(n)$. To get the total error of the network we need to take the sum of the squared errors of all the neurons in the output layer. This can be expressed with the following equation
\[
E(n)=\sum_j \frac{e^2_j(n)}{2}
\]
where $i$ counts all the neurons in the output layer.\\

Our job is now to minimize the cost function, we consider neuron $j$ which receives the input signal and produces the output $v_j$ when we apply the weight on it.
\[
v_j(n) = \sum^m_{i=0}w_{ij}(n)y_i(n)
\]
where $m$ is the number of inputs. The output is passed through the activation function and it appears at the output neuron as
\[
y_j(n)=\varphi_j(v_j(n))
\]
We now take the derivative by using the chain rule and get
\[
\frac{\partial E(n)}{\partial w_{ji}(n)}=\frac{\partial E(n)}{\partial e_j(n)}\frac{\partial e_j(n)}{\partial y_j(n)}\frac{\partial y_j(n)}{\partial v_j(n)}\frac{\partial v_j(n)}{\partial w_{ji}(n)}
\]
\[
=-e_j(n)\varphi_j'(v_j(n)) y_i(n)
\]
Since we are using both sigmoid and the hyperbolic tangent functions as activation functions. Here are the derivatives:
\[
\left(\frac{1}{1+e^{-a v_j(n)}}\right)'=\frac{a e^{-av_j(n)}}{\left(1+e^{-a v_j(n)}\right)^2}
\]
and
\[
(a\text{tanh}(bv_j(n))' = ab\left(1-\text{tanh}^2(bv_j(n))\right)
\]
\subsection{The Delta rule}
We update $w_{ji}(n)$ by applying $\Delta w_{ji}(n)$ which is given by
\begin{equation}
\Delta w_{ji}(n)=-\eta \frac{\partial E(n)}{\partial w_{ji}(n)}=\eta e_j(n) \varphi_j'(v_j(n))y_i(n)
\label{eq:above}
\end{equation}
Using \ref{eq:above} we can rewrite this as
\[
\Delta w_{ji}(n)=\eta \delta_j(n)y_i(n)
\]
where $\delta_j(n)$ is defined as
\[
\delta_j(n)=\frac{\partial E(n)}{\partial v_j(n)}=\frac{\partial E(n)}{\partial e_j(n)}\frac{\partial e_j(n)}{\partial y_j(n)} \frac{\partial y_j(n)}{\partial v_j(n)}=e_j(n)\varphi_j'(v_j(n))
\]


The neuron $j$ could either belong to an output layer and $\delta_j(n)$ can be calculated by the equation above. Or if it belongs to a hidden layer we need to redefine $\delta_j(n)$ where $j$ is the hidden layer. Then $\delta_j(n)$ is
\[
\delta_j(n) = -\frac{\partial E(n)}{\partial y_j(n)}\frac{\partial y_j(n)}{\partial v_j(n)}=-\frac{\partial E(n)}{\partial y_j(n)}\varphi_j'(v_j(n))
\]

When neuron $k$ is an output node then the cost function is given as
\[
E(n)=\sum_k \frac{e^2_k(n)}{2}
\]
When differentiating $E(n)$ w.r.t $y_i(n)$ we get
\[
\frac{\partial E(n)}{\partial y_j(n)}=\sum_k e_k(n)\frac{\partial e_k(n)}{\partial y_j(n)}=\sum_k e_k(n)\frac{\partial e_k(n)}{\partial v_k(n)}\frac{\partial v_k(n)}{\partial y_j(n)}
\]
We can rewrite $e_k(n)$ as before.
\[
e_k(n)=d_k(n)-y_k(n)=d_k(n)-\varphi_k(v_k(n))
\]
When we differentiating $e_k$ w.r.t $v_k$ we have
\[
\frac{\partial e_k(n)}{\partial v_k(n)}=-\varphi_k'(v_k(n))
\]
$v_k=\sum_{j=0}^m w_{kj}y_j(n)$ is the induced local field where m is the number of inputs to node $k$. We are using bias nodes in our model which are set to $+1$. The weights $w_{k0}(n)$ corresponds to the bias terms $b_k(n)$.\\
If we differentiate the error $v_k(n)$ w.r.t $y_j(n)$ we get the weights $w_{kj}(n)$. Using all this we get the partial derivative of the error function $E(n)$ w.r.t $y_j(n)$ which gives us
\[
\frac{\partial E(n)}{\partial y_j(n)}=-\sum_k e_k(n) \varphi_k'(v_k(n))w_{kj}(n)=-\sum_k \delta_k(n)w_{kj}(n)
\]
This gives us the backpropagation formula for the local gradient $\delta_j(n)$ as
\begin{equation} \label{eq:1}
\delta_j(n)=\varphi_j'(v_j(n))\sum_k \delta_k(n)w_{kj}(n)
\end{equation}


In backpropagation algorithm there are two distinct phases. The first phase is the forward phase which means that we apply the forward propagation in order to see if our output data match the computed result from our model. The input passes through the network through the layers until we get an output.\\
The function signal is given by
\[
y_j(n)=\varphi(v_j(n))
\]
and $v_j(n)$ is the so called activation potential of the j:th neuron.
We can write $v_j(n)$ as
\[
v_j(n)=\sum^m_{i=0}w_{ji}(n)y_i(n)
\]
When $j$ is the first hidden layer then $y_i(n)=x_i(n)$ where $x_i(n)$ is the i:th input data to the network. If neuron $j$ is an output node then the output $y_j$ is compared to the target data $d_j(n)$ which gives us the error signal $e_j(n)$.\\
In the backward phase we go recursively through the layers in the network and compute $\delta$ for each neuron in each layer. We update the synaptic weights with the delta rule as we explained before which means that for a neuron in the output layer, the delta value is error multiplied by the first derivate of its activation function. We calculate the changes of all the weights from the output layer to the input layer. When we obtain the delta value from the output layer we calculate the delta for the layer next to the output layer by \ref{eq:1}. This is done recursively through all the layers until a good enough minima is found.




\subsection{Stochastic gradient descent}
Stochastic gradient descent (SGD) is a stochastic approximation of the gradient descent optimization method for minimizing an objective function that is written as a sum of differentiable functions. SGD is looking for minimums or maximums by iteration. To calculate the gradient product may require expensive computation of the gradients from all summand functions. When the training set is large and evaluating the sums of gradients becomes very expensive. To reduce the the computational work at every iteration, SGD samples a subset of at every step. This is very effective when working with larger dataset in machine learning problems.\\
The algorithm performs the updates for each training example. Several passes can be made over the training set until the algorithm converges. If this is done, the data can be shuffled for each pass to prevent cycles.

%The SGD algorithm works as follows:
%\begin{itemize}
%  \item Choose an initial vector of parameters $w$ and learning rate $\eta$.
%  \item Repeat until we find a good enough minima.
%  \item Shuffle the examples in the training set randomly.
%  \item Update $\bar{w}$ according the the algorthim.
%\end{itemize}
%\vspace*{\baselineskip}

Many improvements on the basic SGD algorithm have been proposed and used. Two such variants are Momentum and Adam optimizer.

\subsubsection{Momentum}
Since the gradient descent method is always propagating in straight lines which are perpendicular to the isocurves they often jump back and forth towards a local or global minimum. To improve this course of events we add a term to make the path more smooth towards the minima.
\[
\Delta w(n+1)_{ij}=\alpha \Delta w(n)_{ij}-\eta\frac{\partial E}{\partial w_{ij}}
\]
where E is the cost function, $\alpha$ is a moment coefficient and $\eta$ the learning rate.


\subsubsection{Adam optimizer}
Another variant of stochastic gradient decent is Adaptive moment estimation (Adam). Tests have shown that Adam works well in practice and compares favorably to other adaptive learning method algorithms. It is taking the average of both the gradients and their magnitudes. In addition to storing an exponentially decaying average of past squared gradients $v(w,n)$, Adam also keeps an exponentially decaying average of past gradients $m(w,n)$, similar to the momentum technique. The optimizer is defined as follows with $n$ as the iteration step
\begin{equation}
\begin{gathered}
m(w,n+1)=\gamma_1 m(w,n)+(1-\gamma_1)\nabla E(w,n)\\
v(w,n+1)=\gamma_2 v(w,n)+(1-\gamma_2)\nabla E(w,n)^2\\
\hat{m}(w,n+1)=\frac{m(w,n+1)}{1-\gamma_1^t}\\
\hat{v}(w,n+1)=\frac{v(w,n+1)}{1-\gamma_2^t}\\
\bar{w}(n+1)=\bar{w}(n)-\frac{\eta}{\sqrt{\hat{v}\left(w,n+1\right)}+\epsilon} \hat{m}\left(w,n+1\right)
\end{gathered}
\end{equation}
where $m(w,n+1)$ and $v(w,n+1)$ are estimates of the first and second moment of the gradients respectively. First, $m(w,n)$ and $v(w,n)$ are initialized as vectors of zeros. The algorithm observe that they are biased towards zero, especially during the initial time steps. We set $\gamma_1=0.9$ and $\gamma_2=0.999$ and $\epsilon=10^{-8}$ in similarity to ref \cite{adam}.


\section{K-fold Cross Validation}
We'll utilize the k-fold cross validation for evaluating our models in this project. The idea is to split the dataset into several mutually exclusive and exhaustive subsets. For each split one part will be our validation set and the rest will be used as a training set. This process is done until every single fold has been used as a validation set. By using this method all the data will be used as a validation set without a positive bias. The size of the folds will control the computational bias-variance tradeoff. When using many folds the variance will be lower since the training set will be larger, and when we are using less folds, the variance will be higher since the prediction depends on which fold the samples were assigned. When we are using more folds the computational work will be tougher since we need to train the model more times. The subsets we end up with when doing a k-fold cross validation looks like this

\begin{equation}
\begin{gathered}
\nu_1=\chi_1,\tau_1=\chi_2\cup\chi_3\cup\dots\cups\ci_K\\
\nu_2=\chi_2,\tau_2=\chi_1\cup\chi_3\cup\dots\cups\ci_K\\
\vdots\\
\nu_K=\chi_K,\tau_2=\chi_1\cup\chi_2\cup\dots\cups\ci_{K-1}
\end{gathered}
\end{equation}
\\
\\
where $\nu_i$ is validation set and $\tau_i$ is a training set for $i=1,\dots,K$.


\section{Principal Component Analysis}
The principal component analysis is a tool for extracting relevant information from data sets. It provides a way for to reduce a complex data set to a lower dimensional subspace. We contruct a composite index using uncorrelated components, where each component captures the largest possible variation in the original variables. This could be thought of as an unsupervised version of a multi-output linear regression where we observe the high dimensional response , but not the low dimensional cause.\\
We start by normalize the data so that each dimension have the same magnitude. Then we estimate the covariance matrix. Since the covariance matrix is real and symmetric we can diagonalize it by a orthogonal matrix. We denote the covariance matrix as
\[
C=KDK^T
\]
where K is the orthogonal matrix with columns being eigenvectors corresponding to the eigenvalues of D. And D is the diagonal matrix of eigenvalues. Sort D and K in descending order and we can calculate the total variance of the subspace including the eigenvectors $k_1,\dots,k_n$ by
\[
T_n=\frac{1}{N}\sum^n_{i=1}D_i
\]
N is the number of dimensions of the original data space. $D_i$ is a eigenvalue and $T_n$ the total variance of the linear subspace accounting for the largest amount of variance when using $n$ dimensions.
To get the principal component space we span a space by the $n$ first eigenvectors after they have been sorted by the eigenvalues in descending order. We can choose which $n$ to use by studying how $T_n$ behaves or by just setting an arbitrary threshold for the number of dimensions. In this thesis we use PCA both to visualize the datasets in lower dimensions to evaluate the features and to reduce the number of dimensions.


\section{Stochastic Neighbour Embedding}
Stochastic Neighbor Embedding (SNE) is a technique for dimensionality reduction that is particularly well suited for the visualization of high-dimensional datasets. It starts by converting the high-dimensional Euclidean distances between datapoint into conditional probabilities that represent similarities. While PCA is trying to maximize the variance this algorithm is searching for similarities of data point $x_j$ to datapoint $x_i$. This similarity is expressed with the conditional probability $p_{j|i}$. This means that we get the probability that $x_i$ would pick $x_j$ as its neighbour if neighbours were picked in proportion to their probability density under a Gaussian centered at $x_i$. We can write the conditional probability as
\[
p_{j|i}=\frac{\text{exp}\left(\frac{-||x_i-x_j||^2}{2\sigma_i^2}\right)}{\sum_{k\neq i}\text{exp}\left(\frac{-||x_i-x_k||^2}{2\sigma^2_i}\right)}
\]
Here $\sigma_i$ is the variance of the Gaussian that is on $x_i$. $p_{i|i}$ will be set to zero since we are only looking at the relationship between neighbors. We want to construct a low-dimensional representation of the high-dimensional dataset so we introduce the counterparts of $x_i$ and $x_j$ namely, $y_i$ and $y_j$. We are computing a similar conditional probability we denot by $q_{j|i}$. Here we set the variance of the Gaussian to $\frac{1}{\sqrt{2}}$ to simplify the equation. Hence, we get the conditional probability by

\[
q_{j|i}=\frac{\text{exp}\left(-||y_i-y_j||^2\right)}{\sum_{k\neq i}\text{exp}\left(-||y_i-y_k||^2\right)}
\]
Since we are only interested in the pairwise relationship between different datapoint we set $q_{i|i}$ to zero.
We want to find a state where $p_{j|i}$ is as close to $q_{j|i}$ as possible. Then the new data points $y_j$ and $y_i$ model the similarity between the high dimensional data points $x_j$ and $x_i$. To measure the allegiance of which $q_{j|i}$ models $p_{j|i}$ we use the Kullback-Leibler divergence. We minimize the sum of this divergences over all data points by applying gradient descent. And
\[
C=\sum_i\sum_j p_{j|i}\text{log}\left(\frac{p_{j|i}}{q_{j|i}}\right)
\]
is the cost function which we need to minimize. The gradient is given by
\[
\frac{\partial C}{\partial y_i}=2\sum_j \left(p_{j|i}-q_{j|i}+p_{i|j}-q_{i|j}\right)\left(y_i-y_j\right)
\]
And then we update the $y$ values by taking the gradient with a momentum term.
\[
y(n+1)=y(n)+\eta\frac{\partial C}{\partial y}+\alpha(n)\left(y(n)-y(n-1)\right)
\]
$\alpha$ is the size of the momentum, $y(n+1)$ indicates the solution at iteration n and $\eta$ is the learning rate.


==> include/backmatter/References.tex <==
% CREATED BY ERIK EK, 2016
\begin{thebibliography}{69}

\bibitem{Reference} Rodríguez, G. (2007). Lecture Notes on Generalized Linear Models. URL: \texttt{http://data.princeton.edu/wws509/notes/} [Accessed: 02-November-2016]
\bibitem{Reference} Laurens van der Maaten Visualizing Data using t-SNE (2008) URL: \texttt{https://lvdmaaten.github.io/publications/papers/JMLR2008.pdf} [Accessed: 26-September-2016]
\bibitem{Reference} Ethem Alpaydin Introduction to Machine Learning (2004)
\bibitem{Reference} Kevin P. Murphy Machine Learning - A Probabilistic Perspective (2012)
\bibitem{Reference} Simon Haykin Neural Network - A comprehensive foundation, Second edition (1999)
\bibitem{Reference} Geoffrey Grimmett and David Stirzaker Proabability and Random Processes, Third edition (2001)
\bibitem{Reference} C David. Linear Algebra and its application. Pearson, Third edition (2003)
\bibitem{Reference} I. Goodfellow, Y. Bengio and A. Courville Deep learing (2014) URL: \texttt{http://www.deeplearningbook.org} [Accessed: 20-September-2016]
\bibitem{Reference} I.T. Jolliffe Principal Component Analysis (2002)
\bibitem{Reference} B. Schölkopf, Alexander J. Smola Learning with Kernels: Support Vector Machines, Regularization, Optimization (2002)
\bibitem{Reference}  John A. Rice Mathematical Statistics and Data Analysis, Third edition (2006)
\bibitem{Reference} N. Srivastava, G.Hinton, A.Krizhevsky, I.Sutskever, R.Salakhutdinov Dropout: A Simple Way to Prevent Neural Networks from Overfitting URL: \texttt{https://www.cs.toronto.edu/~hinton/absps/JMLRdropout.pdf} [Accessed: 29-October-2016](2006)
\bibitem{adam} D. Kingma, J.BaAdam: A Method for Stochastic Optimization URL: \texttt{https://arxiv.org/abs/1412.6980} (2014)
\bibitem{Reference} N. Srivastava, G.Hinton, A.Krizhevsky, I.Sutskever, R.Salakhutdinov Dropout: A Simple Way to Prevent Neural Networks from Overfitting URL: 
\texttt{https://arxiv.org/abs/1412.6980} (2014)
\bibitem{relu} X. Glorot, A. Bordes, Y. Bengio DIRO, Universit ee de Montr eeal Deep Sparse Rectifier Neural Networks (2015)
\bibitem{rel1} M. Hippi, I. Juga, A. Rossa, Road weather model development (2010)
\texttt{http://cordis.europa.eu/docs/projects/cnect/5/215455/\\080/deliverables/001-ROADIDEAD34bRoadweathermodeldevelopment1.pdf} [Accessed: 19-September-2016] (2010)
\bibitem{rel2} I. Juga, Pertti N. and M. Hipp, A statistical forecast model for road surface friction (2010)
\texttt{http://www.transport-research.info/sites/default/files/project/\\documents/20120411\_172254\_75532\_15\_sirwec\_2010\_paper\_hippi.pdf} [Accessed: 23-September-2016]
\bibitem{rel3} S. Gupta, J. Funke and T. Lipp, Estimating Road Friction for Autonomous Vehicles
\texttt{http://cs229.stanford.edu/proj2011/\\GuptaFunkeLipp--EstimatingFriction.pdf} [Accessed: 20-September-2016]
\bibitem{rel4} M. Staron and R. Scandariato, Data veracity in intelligent transportation systems: the slippery road warning scenario (2016)
\end{thebibliography}


==> include/extra_points.tex <==
\begin{description}
	\item [{Illustration}] We can use the same method from the following to
	build a method to use the measurements from $t-2T$ to $t-T$ to predict
	the friction level of the road at time $t$. In this case the measurements
	associated with $y_{t}$ is different from the above, in that here
	we are using the measurements till maximum $t-T$ not $t$.
\end{description}
Depending on the goal, different methods can be implemented for the
task. In each case all the available pairs, denoted by $\mathcal{M}=\left\{ (\mathbf{z}_{t},y_{t})\right\} $
are used to train a function $g$ such that 
\[
y_{t}=g\left(\mathbf{z}_{t}\mid M\right)
\]
where $\mid$ is used to show that $M$ is given to design the function.
We consider two cases in the following:


\subsubsection{Classification}

Assume $y_{t}$ is quantized to $K$ levels, e.g., $\left\{ -1,0,1\right\} $
with $K=3$. In this case we can apply classification methods to classify
each vector $\mathbf{z}_{t}$ to one of the $K$ possible classes.
Successful methods for this purpose include support vector machines,
linear discriminant analysis, probabilistic generative models using
mixture distributions, and neural networks.


Binary logistic regression classifier is used for the classification. The binary logistic model is used to estimate the probability of a binary response based on a predictor. In this case will we try to predict if the road is slippery or not. The predicted values are probabilities and are therefore restricted from zero to one through the logistic distribution function because logistic regression predicts the probability of particular outcomes.


\begin{figure}[H]
\centering
\includegraphics[width= \linewidth]{figure/SVM_2.png}
\caption{An example of an support vector machine classifier with soft margin. The hyperplane ($w^Tx+b=0$) is separating the two data classes in these two dimensions with some margin of error.}
\end{figure}

\subsection{Kernel function}
We introduce the kernel function $K(x,x_i)=\phi(x)^T\phi(x_i)$ which only relies on the dot product of the vectors in feature space $F$. When using a kernel it's not necessary to perform an explicit projection to that space as long as the function $K$ has the same results. It can be used instead. This is called the kernel trick. The feature space $F$ can have unlimited dimensions and the hyperplane separating the data can be very complex. This is what gives the SVM its ability to separate non-linear separable data points. One of the popular kernels is the Gaussian Radial Basis function defined as
\[
K(x,x')=\text{exp}\left(-\frac{||x-x'||^2}{2\sigma^2}\right)
\]
$||x-x'||$ is the dissimilarity measure and the $\sigma$ is a kernel parameter. One of the greatest advantages of this method lies in its applicability in almost any dimension because of its versatility. There are generally little restrictions on the way the data are prescribed.


As mentioned in the theory chapter, an neural network can be varied in many ways. For this project we decided to use one hidden layers. The hidden layer contains the same number of nodes as inputs in the input layer. Since we have a smaller training set more layers and nodes would cause overfitting problems. In the next chapter we did an evaluation of how more hidden layers effected the results.\\

\begin{description}
	\item [{Example}] As an example, we use neural networks to design the function
	$g$. Particularly, the system performance can be improved by using
	deep neural networks (DNN). DNN is a machine learning technique that
	uses multiple-layer non-linear transformations to obtain a mapping
	between the input and output data. The standard learning strategy
	consists of randomly initializing the weights of the network and applying
	the gradient descent approach using the back-propagation. In DNN,
	the output $y_{t}$ is produced by non-linear interaction of many
	factors, where these factors are organized into multiple levels, corresponding
	to different levels of abstraction. Varying numbers of layers and
	layer sizes can be used to provide different amounts of abstraction.
	Given the training set $\mathcal{M}$, the DNN is learned and all
	the associated weights are stored. These weights, together with the
	network topology, define the function $g$ such that $y_{t}=g\left(\mathbf{z}_{t}\mid M\right).$
\end{description}

Successful
methods for this purpose include linear regression methods, Gaussian
processes, sparse kernel machines, and statistical methods wit mixture
distributions. 

To predict the friction level of the road at
time $t^{\prime}$, we gather and structure the measurements from
$t^{\prime}-T$ till $t^{\prime}$. We may need to impute the missing
data, as discussed earlier. Then these measurements are stored in
a $df_{s}$-dimensional vector denoted by $\mathbf{z}_{t^{\prime}}$.
The prediction result is now obtained as

\[
y_{t^{\prime}}=g\left(\mathbf{z}_{t^{\prime}}\right).
\]

Feature selection has been performed experimentally and by using cross validation. ... 


\text{Error rate}=\frac{FN+FP}{TP+FP+TN+FN}
\]
In addition to error rate two other measurement were used to assess the results, namely the sensitivity (also called true positive rate) and the specificity (also true negative rate). The sensitivity is defined as
\[
\text{Sensitivity}=\frac{TP}{TP+FN}
\]
which can be described as the number of true positive predictions divided by the number of actual low friction detections. Could also be described as the probability that the model predicts a road segment as slippery given that the segment is slippery.\\
The specificity is defined as
\[
\text{Specificity }=\frac{TN}{TN+FP}
\]
and can be described as the number of true negatives predictions divided by the number of true negatives and the number of false positives. In other words; it measures the proportion of high friction predictions that are correctly identified as such.\\
\\


\begin{table*}[t]
\caption{ ... }
\small{
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\cline{3-8}
\multicolumn{1}{c}{\multirow{2}{*}{}} &  & \multicolumn{3}{c|}{Road Segment 1} & \multicolumn{3}{c|}{Road Segment 2}\\
\cline{3-8}
\multicolumn{1}{c}{\multirow{2}{*}{}} &  & Error rate & Sensitivity & Specificity & Error rate & Sensitivity & Specificity\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{LR}} 
& 0 & 0.2250 & 0.9609 & 0.3361 & 0.2757 & 0.5051 & 0.7823\\
\cline{2-8}
 & 30 & 0.2274 & 0.9312 & 0.4287 & 0.3245  & 0.2556  &0.8474\\
\cline{2-8}
 & 60 & 0.2298 & 0.9668 & 0.2946 & 0.3234 & 0.2000 & 0.8525\\
\cline{2-8}
 & 90 & 0.2406 & 0.9430 &  0.3243 & 0.3271 & 0.1882 &  0.8475\\
\cline{2-8}
 & 120 & 0.2612 & 0.9283 &  0.2857 & 0.3398 & 0.1375 &  0.8428\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{SVM}} 
& 0 & 0.2228 & 0.9358 & 0.4029 & 0.2568& 0.1586 & 0.9568\\
\cline{2-8}
 & 30 & 0.2226 & 0.9305 & 0.4126 & 0.2593& 0.0994 &  0.9725\\
\cline{2-8}
 & 60 & 0.2278 & 0.9295& 0.3915 & 0.2763& 0.0756& 0.9627\\
\cline{2-8}
 & 90 & 0.2330 & 0.9287 & 0.3838 & 0.2551 & 0.1000 & 0.9771\\
\cline{2-8}
 & 120 & 0.2466 & 0.9122& 0.3738 & 0.2558 & 0.0669& 0.9808\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ANN}} 
& 0 & 0.1945& 0.9053 & 0.5526 & 0.2648& 0.4384 &0.8460\\
\cline{2-8}
 & 30 & 0.2130& 0.8760 & 0.5720 & 0.2979& 0.2584 & 0.8621\\
\cline{2-8}
 & 60 & 0.2188& 0.8526& 0.5758 & 0.3054& 0.2649 & 0.8521\\
\cline{2-8}
 & 90 & 0.2299  & 0.8536& 0.5771 & 0.2866  & 0.2276&0.8846 \\
\cline{2-8}
 & 120 & 0.2303 & 0.8632&0.5666 & 0.2847 & 0.3525&0.8427\\
\hline
\end{tabular}
}
\label{final_results}
\end{table*}

==> include/frontmatter/Abstract.tex <==





==> include/frontmatter/Acknowledgements.tex <==
% CREATED BY Erik Ek, 2016
\thispagestyle{plain}			% Supress header
\section*{Acknowledgements}
The work will be carried out as part of the Volvo Cars connected vehicle project.


==> include/frontmatter/Titlepage.tex <==
% CREATED BY Erik Ek, 2016

% COVER PAGE
\begin{titlepage}
\newgeometry{top=3cm, bottom=3cm,
			left=2.25 cm, right=2.25cm}	% Temporarily change margins		
			
% Cover page background 
\AddToShipoutPicture*{\backgroundpic{-4}{56.7}{figure/auxiliary/frontpage_eng.pdf}}
\addtolength{\voffset}{2cm}

% Cover picture (replace with your own or delete)		
%%\begin{figure}[H]
%%\centering
%%\vspace{2cm}	% Adjust vertical spacing here
%%\includegraphics[width=0.9\linewidth]{figure/Wind.png}
%%\end{figure}

% Cover text
\mbox{}
\vfill
\renewcommand{\familydefault}{\sfdefault} \normalfont % Set cover page font
\textbf{{\Huge 	Road Friction Prediction using Machine Learning}} 	\\[0.5cm]
{\Large --}\\[0.5cm]
Master's thesis in Engineering Mathematics and Computational Science \setlength{\parskip}{1cm}

{\Large Erik Ek} \setlength{\parskip}{2.9cm}

Department of Mathematical Sciences \\
\textsc{Chalmers University of Technology} \\
Gothenburg, Sweden 2016

\renewcommand{\familydefault}{\rmdefault} \normalfont % Reset standard font
\end{titlepage}


% BACK OF COVER PAGE (BLANK PAGE)
\newpage
\restoregeometry
\thispagestyle{empty}
\mbox{}


% TITLE PAGE
\newpage
\thispagestyle{empty}
\begin{center}
	\textsc{\large Master's thesis 2016}\\[4cm]		% Report number given by department 
	\textbf{\Large Road Friction Prediction using Machine Learning}\\[1cm]
	{\large Erik Ek}
	
	\vfill	
	% Logotype on titlepage	
	\begin{figure}[H]
	\centering
	% Remove the following line to remove the titlepage logotype
	\includegraphics[width=0.2\pdfpagewidth]{figure/auxiliary/logo_eng.pdf} \\	
	\end{figure}	\vspace{5mm}	
	
	Department of Mathematical Sciences \\
	\emph{-}\\
	\textsc{Chalmers University of Technology} \\
	Gothenburg, Sweden 2016 \\
\end{center}


% IMPRINT PAGE (BACK OF TITLE PAGE)
\newpage
\thispagestyle{plain}
\vspace*{4.5cm}
Road Friction Prediction using Machine Learning\\
ERIK EK \setlength{\parskip}{1cm}

\copyright ~ ERIK EK, 2016. \setlength{\parskip}{1cm}

Supervisor: Mats Rudemo, Mathematical Statistics, Chalmers\\
Supervisor: Ghazaleh Panahandeh, Sensor Fusion, Volvo Cars\\
Examiner: Mats Rudemo, Mathematical Statistics, Chalmers \setlength{\parskip}{1cm}

Master's Thesis 2016\\\\	% Report number given by department 
Department of Mathematical Statistics\\
Chalmers University of Technology\\
SE-412 96 Gothenburg\\
%Telephone +46 31 772 1000 \setlength{\parskip}{0.5cm}

Sensor Fusion\\
Volvo Car Corporation\\
SE-412 96 Gothenburg\\
%Telephone +46 31 772 1000 \setlength{\parskip}{0.5cm}

\vfill
% Caption for cover page figure if used, possibly with reference to further information in the report
\setlength{\parskip}{0.5cm}

Typeset in \LaTeX \\
%Printed by [Name of printing company]\\
Gothenburg, Sweden 2016



==> include/missingData.tex <==
\subsection{Structuring Measurements}

The number of passing cars in a street or road might significantly vary depending on the weather condition, road connections etc, which means that the number of received measurements also vary. A related issue arises when the distribution of the passing cars during the
desired interval, e.g., one hour, is different over time. In other
words, tens of measurements might be received from 30 minutes ago
until 15 minutes ago, while no measurements be received from 15 minutes
ago until the current time. The missing measurements, i.e., the ones
that we have not received during the desired interval, provide a complication
in the prediction.
These issues lead to inhomogeneous structure in
the input data, and this has to be corrected before processing. 
We define a reference sampling rate for the measurements, which can
be street-dependent. This number should be set proportional to the
number of cars passing from the street. Additionally, we only use
a limited number of past measurements, the measurements received in
the desired interval which can be, e.g., 1 hour, to perform the prediction.
Let $T$ denote the desired interval, such that all the measurement
from $t-T$ until $t$ are used to predict an output for time $t$.
Also denote the reference sampling rate by $f_{s}$. The goal of ``structuring
measurements'' is to create a feature vector from all the measurements
obtained from $t-T$ until $t$. As discussed above, there might be
many or just a few measurements in this interval. We re-sample the
number of measurements such that only $f_{s}$ measurements are available
$t-T$ until $t$. Consider two cases:
\begin{itemize}
	\item Down-sampling: When there are many measurements we need to down-sample.
	This is intuitive because the received measurements are highly correlated. 
	\item Missing-data: If there is not enough measurement, we mark that portion
	of data as missing (see the later sections).\end{itemize}
\begin{description}
	\item [{Example}] Assume $T=60$ minutes, and $f_{s}=60$. Hence, we structure
	the measurements such that we have one measurement in each minutes
	in the last 60 minutes. If there are measurement in some minutes,
	we only keep one of them and throw away the others. If we do not have
	any measurement for some minutes, we mark the corresponding measurements
	as missing. This is done during both training and testing. 
\end{description}
Assume the dimension of measurement vector in each time is $d$. We
have $f_{s}$ number of measurements each being $d$-dimensional that
can be used to predict an output. These measurement are stored in
a $d\times f_{s}$ matrix (in which some of the columns are unknown),
which is denote by $\mathbf{x}_{t}$, where $t$ denotes the time. 

\subsection{Handling Missing Data}
There are various ways to handle the missing data for classification
or prediction. Denote the observed and missing part of $\mathbf{x}_{t}$
by $\mathbf{x}_{t,obs}$ and $\mathbf{x}_{t,miss}$, respectively.
In general, a function $f$ is designed such that
\[
\mathbf{x}_{t,miss}=f\left(\mathbf{x}_{t,obs}\mid\mathbf{X}_{obs}\right)
\]
where $\mathbf{X}_{obs}$ represents all the available (observed)
measurements. Imputation methods based on K-nearest neighbor (K-nn)
method and multi-layer perceptron imputation can be used to design
$f$. In the current application, a very effective solution for this
problem can be designed since each column of $\mathbf{x}_{t}$ represent
a similar set of measurements, which are also very correlated with
the neighboring measurements. For example, if no measurement is available
at a given time, we can use the measurements from neighboring times
to impute the missing measurement. More formally, let $\tau$ denote
the index of the missing measurement in $\mathbf{x}_{t}$, so that
that $\tau-th$ column of $\mathbf{x}_{t}$ ($\mathbf{x}_{t,\tau}$)
is missing. We design the function $f$ as follows to estimate the
missing data:

\[
\mathbf{x}_{t,\tau}\approx f\left(\mathbf{x}_{t}\right)=\sum_{m=1}^{f_{s}}\alpha_{m}\left(\tau\right)\mathbf{x}_{t,m}
\]
where $\alpha_{m}\left(\tau\right)$ defines the weights. Many choices
are possible for this purpose. 
\begin{description}
	\item [{Example1}] We can use only the measurement before and after $\tau$
	to estimate $\mathbf{x}_{t,\tau},$ leading to:
\end{description}
\[
\alpha_{m}\left(\tau\right)=\begin{cases}
\begin{array}{c}
0.5\\
0
\end{array} & \begin{array}{c}
m=\tau-1,m=\tau+1\\
otherwise
\end{array}\end{cases}
\]

\begin{description}
	\item [{Example2}] We can use all the columns of $\mathbf{x}_{t},$ leading
	to
\end{description}
\[
\alpha_{m}\left(\tau\right)=\frac{a}{\left|m-\tau\right|},
\]
where $\left|\cdot\right|$is the absolute value, and $a$ is such
that $\sum_{m}\alpha_{m}\left(\tau\right)=1$.

After estimating a value for the missing measurement, the missing
part is replaced with the estimate quantity to obtain full measurement
$d\times f_{s}$-dimensional matrix $\mathbf{x}_{t}$. To perform
the prediction, we vectorized this measurement matrix to obtain a $df_{s}$-dimensional
vector denoted by $\mathbf{z}_{t}$.

==> include/settings/Settings.tex <==
% CREATED BY DAVID FRISK, 2016

% BASIC SETTINGS
\usepackage{moreverb}								% List settings
\usepackage{textcomp}								% Fonts, symbols etc.
\usepackage{lmodern}								% Latin modern font
\usepackage{helvet}									% Enables font switching
\usepackage[T1]{fontenc}							% Output settings
\usepackage[english]{babel}							% Language settings
\usepackage[utf8]{inputenc}							% Input settings
\usepackage{amsmath}								% Mathematical expressions (American mathematical society)
\usepackage{amssymb}								% Mathematical symbols (American mathematical society)
\usepackage{graphicx}								% Figures
\usepackage{subfig}									% Enables subfigures
\numberwithin{equation}{chapter}					% Numbering order for equations
\numberwithin{figure}{chapter}						% Numbering order for figures
\numberwithin{table}{chapter}						% Numbering order for tables
\usepackage{listings}								% Enables source code listings
\usepackage{chemfig}								% Chemical structures
\usepackage[top=3cm, bottom=3cm,
			inner=3cm, outer=3cm]{geometry}			% Page margin lengths			
\usepackage{eso-pic}								% Create cover page background
\newcommand{\backgroundpic}[3]{
	\put(#1,#2){
	\parbox[b][\paperheight]{\paperwidth}{
	\centering
	\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
\usepackage{float} 									% Enables object position enforcement using [H]
\usepackage{parskip}								% Enables vertical spaces correctly 



% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)

% Disable automatic indentation (equal to using \noindent)
\setlength{\parindent}{0cm}                         


% Caption settings (aligned left with bold name)
\usepackage[labelfont=bf, textfont=normal,
			justification=justified,
			singlelinecheck=false]{caption} 		

		  	
% Activate clickable links in table of contents  	
\usepackage{hyperref}								
\hypersetup{colorlinks, citecolor=black,
   		 	filecolor=black, linkcolor=black,
    		urlcolor=black}


% Define the number of section levels to be included in the t.o.c. and numbered	(3 is default)	
\setcounter{tocdepth}{5}							
\setcounter{secnumdepth}{5}	


% Chapter title settings
\usepackage{titlesec}		
\titleformat{\chapter}[display]
  {\Huge\bfseries\filcenter}
  {{\fontsize{50pt}{1em}\vspace{-4.2ex}\selectfont \textnormal{\thechapter}}}{1ex}{}[]


% Header and footer settings (Select TWOSIDE or ONESIDE layout below)
\usepackage{fancyhdr}								
\pagestyle{fancy}  
\renewcommand{\chaptermark}[1]{\markboth{\thechapter.\space#1}{}} 


% Select one-sided (1) or two-sided (2) page numbering
\def\layout{2}	% Choose 1 for one-sided or 2 for two-sided layout
% Conditional expression based on the layout choice
\ifnum\layout=2	% Two-sided
    \fancyhf{}			 						
	\fancyhead[LE,RO]{\nouppercase{ \leftmark}}
	\fancyfoot[LE,RO]{\thepage}
	\fancypagestyle{plain}{			% Redefine the plain page style
	\fancyhf{}
	\renewcommand{\headrulewidth}{0pt} 		
	\fancyfoot[LE,RO]{\thepage}}	
\else			% One-sided  	
  	\fancyhf{}					
	\fancyhead[C]{\nouppercase{ \leftmark}}
	\fancyfoot[C]{\thepage}
\fi


% Enable To-do notes
\usepackage[textsize=tiny]{todonotes}   % Include the option "disable" to hide all notes
\setlength{\marginparwidth}{2.5cm} 


% Supress warning from Texmaker about headheight
\setlength{\headheight}{15pt}		




